Mixed Hodge structures in log symplectic geometry

We study the cohomology rings of snc log symplectic pairs $(X,Y)$ which have log symplectic forms of pure weight. We show that under a certain natural condition, the cohomology ring of $X \setminus Y$ exhibits the curious hard Lefschetz property. Analogous results are shown to hold for limit mixed Hodge structures associated to good degenerations of projective irreducible holomorphic symplectic manifolds. We provide several examples of log symplectic pairs of pure weight including a class of cluster-type varieties, and examples coming from the work of Feigin and Odesski. We show that the components of the central fiber of good degenerations of projective irreducible holomorphic symplectic manifolds produce log symplectic pairs.

==> Consequences.tex <==
\section{Consequences}

In this section, we will explain the geometric consequences of Theorems \ref{thm:ehl} and \ref{thm:chl} in the geometric contexts considered in earlier sections of this article. In the case of good degenerations, this manifests as evidence for Nagai's conjecture. In the case of log symplectic pairs, this manifests as a strict classification of the possible Hodge diamonds of the corresponding pairs.



==> LongModifications.tex <==
\subsection{Blowing up symplectic leaves}\label{sect:leafblow}

The goal of this section is to explain how one can produce new examples of log symplectic varieties from known examples. This implies that unlike the case of compact holomorphic symplectic manifolds, we can produce {\em many} families of log symplectic varieties once we are able to produce a single example. In particular, the examples in Section \ref{sect:purel} can be used to produce a host of new examples by appropriate blow up. 
\begin{comment}
We will now establish notation that will be used repeatedly in this section. Let $\sigma$ be a log symplectic form on $X$ with log poles on $Y$. We let $Y_1,\dots, Y_k$ denote the irreducible components of $Y$. For each subset $I \subseteq \{1,\dots, k\}$ we will let $Y_I = \cap_{i\in I}Y_i$. Then $\partial Y_i = \cup_{i \in I, I \neq \{i\}} Y_I$. For each $Y_i$ we may take the residue of $\sigma$ on $Y_i$ which we denote $\mathrm{Res}_{Y_i}(\sigma)$. If we let $\partial Y_i$ be the union of the intersections of $Y_i$ with all $Y_j$ with $j \neq i$, then $\mathrm{Res}_{Y_i}(\sigma) \in \HH^0(Y_i, \Omega_{Y_i}^1(\log \partial Y_i))$. 

Assume that $V$ is a smooth subvariety of $Y_i$ which intersects the components of $\partial Y_i$ transversally. We may construct the pair $(\mathrm{Bl}_V X, Y_V)$ where $Y_V$ is the proper transform of $Y$ under the blow up map $b_V: \mathrm{Bl}_VX \rightarrow X$. We will show that $(\Bl_VX, Y_V)$ is again log symplectic if $V$ is a nice enough subvariety of $Y_i$, as determined by the behaviour of $\mathrm{Res}_{Y_i}(\sigma)$.

We make the following collection of local observations which may be checked easily in local coordinates.
\begin{proposition}\label{prop:local}
Let $Y_1,\dots, Y_k$ be divisors in a smooth variety $X$ which intersect transversally at a point $p$. 
\begin{enumerate}
\item[1.] If $V$ is a smooth codimension 1 subvariety of $Y_1$ which intersects each $Y_I$ transversally, then $Y_V$ is simple normal crossings in $\Bl_V X$.
\item[2.] If $V'$ is a smooth codimension 1 subvariety of $Y_2$ and $V \cap Y_I$ and $V' \cap Y_I$ intersect transversally for all $I$, then $b_V^{-1}(V')$ intersects $Y_V$ transversally in $\Bl_VX$.
\item[3.] If $V'$ and $V''$ are smooth codimension 1 subvarieties of $Y_2$ and $Y_3$ respectively so that $V \cap Y_I$, $V'\cap Y_I$, and $V'' \cap Y_I$ intersect pairwise transversally for all $I$, then $b_V^{-1}(V') \cap Y_{V,I}$ and $b_V^{-1}(V'')\cap Y_{V,I}$ intersect transversally in $Y_{V,I}$ for all $I$.
\end{enumerate}
\end{proposition}
\end{comment}
\noindent It will be important to have a nice local form for $\sigma$ near smooth points of $Y_i$. Such an expression is supplied by Goto.
\begin{lemma}[{Goto \cite[Lemma 1-2]{goto}}]\label{prop:darboux}
Let $(X,Y)$ be log symplectic with $\dim X = 2d$ and let $p$ be a smooth point in $Y$. Then there are holomorphic coordinates $x_1,\dots, x_{2d}$ near $p$ so that 
\[
\sigma = \dfrac{dx_1}{x_1} \wedge dx_2 + dx_3 \wedge dx_4 + \dots + dx_{2d-1} \wedge dx_{2d}.
\]
\end{lemma}
\noindent We will refer to coordinates in which $\sigma$ has the form of Lemma \ref{prop:darboux} as {\em log holomorphic Darboux coordinates}. If $(X,Y)$ is a log symplectic pair, then the log symplectic form $\sigma$ induces an isomorphism
\[
\mathscr{T}_X(-\log Y) \longrightarrow \Omega_X(\log Y)
\]
Therefore $\sigma$ is equivalent to a holomorphic bivector field $\sigma' \in \HH^0(X,\wedge^2\mathscr{T}_X(-\log Y))$, which gives rise to a map
\[
\Omega_X(\log Y) \longrightarrow \mathscr{T}_X(-\log Y).
\]
We note that $\mathscr{T}_X(-\log Y)$ is a subsheaf of $\mathscr{T}_X$, therefore, this map can be extended to a homomorphism from $\Omega_X(\log Y)$ to $\mathscr{T}_X$ which is, of course, no longer an isomorphism.
\begin{defn}
Let $Z$ be a compact subvariety of $X$, We say that $Z$ is a closed symplectic leaf of $(X,Y)$ if at each point $p$ in a Zariski open dense subset of $Z$, the image of the map
\[
\Omega_X(\log Y)_p \longrightarrow \mathscr{T}_{X,p}
\]
coincides with $i_*\mathscr{T}_{Z,p}$.
\end{defn}
\noindent The following result is an easy consequence of Proposition \ref{prop:darboux}. 
\begin{proposition}
Assume that $Z$ is a smooth subvariety of $X$ of codimension 2 which is contained in some irreducible component $Y_i$ of $Y$. Then $Y$ is a closed symplectic leaf if and only if $\mathrm{Res}_{Y_i}(\sigma)|_Z = 0$.
\end{proposition}
\noindent The following is a generalization of a result appearing in work of Hacking and Keel \cite{hk}.


\begin{proposition}\label{prop:hackingkeel}
Let $(X,Y)$ log symplectic pair with log symplectic form $\sigma$ and let $V$ be a closed symplectic leaf of $\sigma$ of codimension 2 in $X$, which is contained in $Y_1$ and which intersects all strata $Y_I \subseteq Y_1$ transversally. Then $(\mathrm{Bl}_VX,Y_V)$ is log symplectic with symplectic form $\pi_V^*\sigma$.
\end{proposition}
\begin{proof}
This is a local computation, so we restrict ourselves to local charts in $X$. Let us choose some open polydisc $D$ in $X$ centered at a smooth point $p$ in $Y$ which contains $Z$, and let us assume that we have chosen a Darboux coordinate system (Proposition \ref{prop:darboux}), so that
\[
\sigma = d\log x_1\wedge dx_2 + \dots  + dx_{2d-1} \wedge d x_{2d}.
\]
In this coordinate system we have that $Y_1 = Z(x_1)$. Then $\mathrm{Res}(\sigma) = dx_2$, so $V = Z(x_1,x_2)$ in these coordinates. Now we will blow up $X$ in $V$ and show that $\pi^*_V\sigma$ remains log symplectic. The blow up is covered by two charts
\[
U_1 = \{ x_1t = x_2 \} \in D \times \mathbb{C}_{t}, \qquad U_2 = \{ x_1 = x_2s \} \in D \times \mathbb{C}_{s}.
\]
In $U_1$, the proper transform of $x_1 = 0$ does not intersect the exceptional divisor, and in $U_2$, the proper transform of $x_1 = 0$ is given by $s = 0$. In $U_1$, $\pi^*_V\sigma$ is written as
\begin{align*}
b^*_V\sigma|_{U_1} &= d\log x_1 \wedge (x_1d t + t d x_1) + \dots + dx_{2d-1} \wedge d x_{2d} \\
& =  dx_1 \wedge d t + \dots + dx_{2d-1} \wedge d x_{2d}
\end{align*}
and in $U_2$, $\pi^*_V\sigma$ is written as
\[
b^*_V\sigma|_{U_2} = d\log s \wedge d x_2 + \dots + dx_{2d-1} \wedge d x_{2d}.
\]
Therefore, $b^*_V\sigma |_{C_1}$ and $b^*_{V}\sigma|_{C_2}$ are expressed in holomorphic and log holomophic Darboux coordinates respectivey and thus $b^*_V\sigma$ is nondegenerate everywhere in the preimage of a Zariski open subset of $V$. Since near a point outside of $V$, $b_V$ is the identity, we also have that $b_V^*\sigma$ has log poles and is nondegenerate everywhere except at points which are in the preimage of the intersection of $V$ and components $Y_2,\dots, Y_k$. We also note that $b_V^*\sigma$ has non-trivial log poles along each component of $Y_V$.

By the assumption the intersection of $V$ with each $Y_I$ is normal crossings, it follows that $Y_V$ is also normal crossings by Proposition \ref{prop:local}(1). Similarly, this also means that $b^*_V\sigma$ has log poles at $Y_V$. Points in $\Bl_VX$ which are in the preimage of $V\cap \partial Y_1$ form a subset of codimension at least 2 in $\Bl_VX$. Therefore, since degeneracy occurs along a divisor (which is determined locally by the vanishing of the Pfaffian of $b^*_V\sigma$), it follows that $b_V^*\sigma$ is nondegenerate anywhere in $\Bl_VX$, hence $(\Bl_VX,Y_V)$ is log symplectic with log symplectic form $b^*_V\sigma$.
\end{proof}


\begin{remark}
Therefore, if we have a log symplectic pair, we can construct new log symplectic pairs by understanding the residues of $\sigma$ on components of $Y$, and by understanding the compact leaves of the corresponding foliation. According to Goto \cite[Lemma 1-3]{goto}, if $V$ is a submanifold of $Y^\mathrm{sm}$ so that $\mathrm{Res}(\sigma)|_V = 0$, then $V$ is holomorphic symplectic.
\end{remark}
\begin{comment}
\noindent We may of course expand on the construction of $(\Bl_VX,Y_V)$ given above. For each $i \in \{1,\dots, k\}$, let us choose $\{V_{i,1},\dots, V_{i,\ell_i}\}$ where each $V_{i,j}$ is a codimension 1 subvariety of $Y_i$ for which $\mathrm{Res}_{Y_i}(\sigma)|_{V_{i,j}} = 0$. Let us also assume that $V_{i,1},\dots, V_{i,\ell_i}$ are all disjoint and that their intersection with each $Y_I$ is transverse. Furthermore, assume that for all $i \neq j$,$V_{i,m} \cap Y_I$ and $V_{j,n} \cap Y_I$ intersect transversally for all $m,n$ and $I$. Let $\bm{V}$ denote the collection of all $V_{i,j}$. Define $b_{\bm{V}}: \Bl_{\bm{V}} X \rightarrow X$ to be the iterated blow up of $X$ along $V_1,\dots, V_\ell$ (that is, the blow up of $X$ in $V_{1,2}$, followed by the blow up of $\Bl_{V_{1,1}}X$ in the proper transform of $V_{1,2}$ etc.). Let $Y_{\bm{V}}$ be the proper transform of $Y$ under $b_{\bm{V}}$. 
\end{comment}

\begin{corollary}\label{cor:iteratedblow}
Let notation be as above. Then $(\Bl_{\bm{V}}X,Y_{\bm{V}})$ equipped with the form $b_{\bm{V}}^*\sigma$ is an snc log symplectic pair.
\end{corollary}
\begin{proof}
Assume, that $V_{1,1}$ is the element of $\bm{V}$ that we have chosen to blow up first. We have chosen the remaining $Y_{i,m}$ and $Y_{j,n}$ so that $Y_{i,m} \cap Y_I$ and $Y_{j,n}\cap Y_I$ intersect transversally in $Y_I$. Therefore, Proposition \ref{prop:local}(3) implies that their proper transforms intersect each other transversally in all strata as well, and by Proposition \ref{prop:local}(2), they intersect each stratum in the proper transform of $Y$ transversally too. 

Since the residue map is defined locally, and the blow up map $b_{V_{1,1}}$ only affects each $V_{i,m}$ away from a set of codimension 2, it follows that $\mathrm{Res}_{Y_1}(b_{V_{1,1}}^*\sigma)|_{V_{i,m}} = 0$ for all $i,m \neq 1,1$. Therefore, the collection of proper transforms of subvarieties in $\bm{V} \setminus V_{1,1}$ in the pair $(\Bl_{V_{1,1}}X,Y_{V_{1,1}})$ have the same properties with respect to $b_{\bm{V}}^*\sigma$ as the collection $\bm{V}$ in $(X,Y)$ has with respect to to the form $\sigma$. Therefore, the result follows by iterating this procedure.
\end{proof}

\begin{proposition}\label{prop:purity}
If $(X,Y)$ is pure of weight $w$ and $\bm{V}$ is as above, then $(\Bl_{\bm{V}}X,Y_{\bm{V}})$ is also pure of weight $w$.
\end{proposition} 
\begin{proof}
Corollary \ref{cor:iteratedblow} is proved by iterating the procedure in Proposition \ref{prop:hackingkeel}, so it is enough to show that the proposition is true for a single codimension 1 subvariety $V$ in $Y_1$ which intersects each $Y_I$ transversally, with the property that $\mathrm{Res}_{Y_1}(\sigma)|_V = 0$.

Let $E_V$ be the intersection of $\Bl_VX \setminus Y_V$ and the exceptional divisor of $b_V$. We begin by noticing that $b_V|_{\Bl_VX \setminus (Y_V \cup E_V)}$ is a biholomorphic map with image $X \setminus Y$. We will use the notation $\iota$ to denote its inverse composed with the open embedding of $\Bl_VX \setminus (Y_V \cup E_V)$ into $\Bl_V X \setminus Y_V$.


We would like to show that the map $\iota^* : \HH^2(\Bl_VX \setminus Y_V) \rightarrow \HH^2(X \setminus Y)$ is injective on $F^2$, and that this map sends the class represented by $\iota^*\sigma$ to the class represented by $\sigma$. If we can show these two things, then the result comes from the following argument. The map $\iota^*$ induces a morphism of mixed Hodge structures. A morphism of mixed Hodge structures between $(V_1,F_1,W_2)$ and $(V_2, F_2,W_2)$ sends $I^{2,w}(V_1)$ to $I^{2,w}(V_2)$ and agrees with the induced morphism on Hodge and weight graded pieces, therefore, the induced maps $I^{2,i}(\HH^2(\Bl_VX \setminus Y)) \rightarrow I^{2,i}(\HH^2(X \setminus Y))$ are injective for each $i$. We can represent $[\iota^*\sigma]$ uniquely as a sum of classes $\sigma_{2,0} + \sigma_{2,1} + \sigma_{2,2}$ where $\sigma_{2,i} \in I^{2,i}(\HH^2(\Bl_V X \setminus Y_V))$. Since $\iota^*$ is injective on each summand and $[\sigma]$ is pure of weight $w$ for some $w \in \{0,1,2\}$, it follows that $\sigma_{2,i} = 0$ for $i \neq w$.

We start by showing that the pullback map $\HH^2(\Bl_VX \setminus Y_V) \rightarrow \HH^2(X\setminus Y)$ is injective on $F^2$, or equivalently, that the map $\HH^{2d-2}_c(X \setminus Y) \rightarrow \HH^{2d-2}_c(\Bl_VY\setminus Y_V)$ is surjective in $\Gr_F^{2d-4}$. By construction, we have that $X \setminus Y$ is a Zariski open subset of $\Bl_V Y \setminus Y_V$, and its complement is $E_V$, an $\mathbb{A}^1$ bundle over $V$. We have a long exact sequence of mixed Hodge structures,
\[
\dots \longrightarrow \HH^i_c(X \setminus Y) \longrightarrow \HH^i_c(\Bl_VY \setminus Y_V) \longrightarrow \HH^i_c(E_V) \longrightarrow \dots 
\]
The mixed Hodge structure on $\HH^{2d-2}_c(E_V)$ is dual to that of $\HH^0(E_V)$, therefore, it is isomorphic to $\mathbb{Q}(2-d)$, hence $\Gr_F^{2d-4}\HH^2(E_V) = 0$, and it follows that the induced map $\Gr_F^{2d-4}\HH^{2d-2}_c(X \setminus Y) \rightarrow \Gr_F^{2d-4}\HH^{2d-2}(\Bl_VY \setminus Y_V)$ is surjective. By duality, we obtain the desired injectivity.  

Now $[\iota^*\sigma]$ induces a class in $F^2\HH^{2}(\Bl_VX \setminus Y_V)$, via the quasi-isomorphism
\[
\mathscr{A}^\bullet_{\Bl_VX}(\log Y_V) \hooklongrightarrow \mathscr{A}^\bullet_{\Bl_VX \setminus Y_V}
\]
obtained by pullback, and the fact that $\iota^*\sigma$ is closed. The map $\HH^i(\Bl_VX \setminus Y_V) \rightarrow \HH^i(X \setminus V)$ is a morphism of mixed Hodge structure and is induced, again, by pullback on forms,
\[
\mathscr{A}^\bullet_{\Bl_V X \setminus Y_V} \longrightarrow \mathscr{A}^\bullet_{X\setminus Y}
\]
so that class represented by $b^*\sigma$ in $\HH^2(\Bl_VX \setminus Y_V)$ is identified with the class of $\sigma$, since $\iota$ is an isomorphism away from the exceptional divisor $E_V$. This proves the result.
\end{proof}
\begin{example}[Blow ups of the Feigin--Odesski example]
In the Feigin--Odesski examples, the snc log symplectic compactification described in Section \ref{sect:purel} has boundary composed of a pair of divisors, both of which are fiber bundles over a product of elliptic curves. The symplectic leaves of this Poisson structure are $\mathbb{P}^1$-bundles over factors of this product of elliptic curves. We may then produce an infinite number of examples of log symplectic pairs of pure weight 1 and dimension 4 by the process described in this section. In Corollary \ref{cor:noprod}, we showed that this example is not a product of log symplectic pairs of dimension 2; is the Feigin--Odesski example related to a product of log symplectic surfaces by blowing up leaves?
\end{example}
\begin{example}[Cluster varieties]\label{ex:cluster}
Let $N$ be lattice of rank $2d$, and let $\Sigma$ be a rational, complete fan inside of $M \otimes \mathbb{R}$, so that each cone $C$ of $\Sigma$ has generators which generate $\mathrm{span}(C) \cap M$. Then the associated toric variety $X_\sigma$ is smooth. Let $\alpha$ be a holomorphic 2-form on $\mathbb{C}^{*2d}$ of the form
\[
\alpha = \sum_{1\leq i< j\leq 2d} a_{ij} d\log x_i\wedge d\log x_j
\]
and assume that the alternating matrix $A=[a_{ij}]$ is nondegenerate. It is well known that $\alpha$ extends to a log symplectic form on the pair $(X_\Sigma, Y_\Sigma)$ where $Y_\Sigma$ is the union of the torus orbits in $X_\Sigma$ of dimension $\leq 2d-1$.

Let $\bm{Z} = \{Z_1,\dots, Z_k\}$ be symplectic leaves of the Poisson structure on $X_\Sigma$ induced by $\alpha$, and assume that for each codimension 2 torus orbit, $T$ of $X_\Sigma$, and for all $i\neq j$ $Z_i \cap T$ and $Z_j$. Then we may repeatedly blow up along $Z_1,\dots, Z_j$ to obtain a new log symplectic pair $X_{\Sigma, \bm{Z}}$. The variety $U_{\Sigma,\bm{Z}} :=X_{\Sigma,\bm{Z}} \setminus Y_{\Sigma,\bm{Z}}$ is called a {\em cluster variety} by Hacking and Keel \cite{hk}; we will use the term {\em toric cluster pair} to refer to the pair $(X_{\Sigma,\bm{Z}}, Y_{\Sigma,\bm{Z}})$, and the term {\em toric cluster variety} to refer to $U_{\Sigma,\bm{Z}}$.
\end{example}
\begin{remark}
In dimension 2, a result of Gross, Hacking, and Keel \cite{ghk} shows that all pure weight 2 log symplectic pairs are cluster log symplectic. For pure weight 1 log symplectic pairs, one may use results of Friedman and Miranda \cite{fm} to see that there are three families of log symplectic pairs from which one may obtain all pure weight 1 log symplectic pairs by applying Proposition \ref{prop:hackingkeel}, namely, $(\mathbb{P}^2,E)$, $(\mathbb{P}^1\times \mathbb{P}^1, E)$ (for $E$ a smooth anticanonical elliptic curve), and $(\mathbb{P}^1\times E, \{0,\infty\} \times E)$. In higher dimensions, can one find a finite number of ``seed'' log symplectic pairs from which all other log symplectic pairs can be obtained?
\end{remark}
\begin{theorem}\label{thm:cluster}
Let $U_{\Sigma,\bm{Z}}$ be toric cluster variety, then the cohomology ring $\HH^*(U_{\Sigma,\bm{Z}};\mathbb{Q})$ has the curious hard Lefschetz property.
\end{theorem}
\begin{proof}
By Proposition \ref{prop:purity}, $(X_{\Sigma,\bm{Z}}, Y_{\Sigma,\bm{Z}})$ is a log symplectic pair of pure weight 2. The result then follows from Corollary \ref{cor:scr-geom}.
\end{proof}

\begin{remark}\label{rmk:ls}
A similar result is proven by Lam and Speyer \cite{ls}, but their result differs from ours in both technique and scope. The authors of \cite{ls} deal with cluster varieties with the so-called Louise property, which means that they admit a nice cover by acyclic cluster varieties. In \cite{ha2}, we will show that acyclic cluster varieties are toric cluster varieties, but cluster varieties with the Louise property are not generally toric cluster varieties, hence our results do not suffice to recover theirs except in the acyclic case. On the other hand, toric cluster varieties need not be cluster varieties in the traditional sense at all, therefore, Theorem \ref{thm:cluster} does not follow from the results of \cite{ls} either.
\end{remark}




\begin{comment}
\subsection{Symplectic quotients and vlog symplectic pairs}

Given a symplectic pair $(X,Y)$, we may study the cohomology of finite quotients of $X$ which preserve $Y$. We say that a subgroup of $\mathrm{GL}_n(\mathbb{C})$ is small if no element has 1 as an eigenvalue of multiplicity $n-1$. 
\begin{defn}
Let $X$ be an analytic space; we say that $X$ is a $V$-manifold if it has a covering made up of charts analytically isomomrphic to $Z/G$ where $Z$ is an open ball in $\mathbb{C}^n$ and $G$ is a small, finite subgroup of $\mathrm{GL}_n(\mathbb{C})$ which fixes $Z$.
\end{defn}
The condition that the groups $G$ be small ensures that the singular locus of $G$ has codimension at least 2.

Steenbrink \cite{steen} studies the cohomology theory of projective $V$-manifolds; in particular, he shows that their cohomology behaves exactly as the cohomology of a smooth projective variety. Let $\Sigma$ be the singular locus of a V-manifold $X$, and $j : X \setminus \Sigma \hookrightarrow X$ the open inclusion. Then we may let $\widetilde{\Omega}^\bullet_X = j_*\Omega_X^\bullet$. Then \cite[Corollary 1.9]{steenorb} says that $\widetilde{\Omega}^\bullet_X$ is a resolution of the constant sheaf, and that the Hodge-to-de Rham spectral sequence for $\widetilde{\Omega}_X^\bullet$ degenerates at the $E_1$ term to $\HH^{p+q}(X;\mathbb{C})$. 
\begin{defn}
A divisor $Y$ in a V-manifold $X$ is V-normal crossings if $X$ is a V-manifold, and for each orbifold chart $Z/G$ the preimage of $Z/G \cap Y$ in $Z$ is normal crossings.
\end{defn}
Then, in the same way, we may analyze the Hodge theory of V-normal crossings pairs. We define
\[
\widetilde{\Omega}^\bullet_X(\log Y) = j_*\Omega^\bullet_{X\setminus \Sigma}(\log(Y \setminus \Sigma))
\]
In local charts, $\widetilde{\Omega}^\bullet_X(\log Y) = (\rho_*\Omega_Z^\bullet(\log D))^G$. On the complex, $\widetilde{\Omega}_X^\bullet(\log Y)$, we may define weight and Hodge filtrations $W_\bullet, F^\bullet$ as in Section \ref{sect:mhs}. As a consequence of \cite[Theorem 1.12, Lemma 1.19]{steenorb}, the bifiltered complex $(\widetilde{\Omega}_X^\bullet(\log Y), F, W)$ may be used to compute the canonical mixed Hodge structure on $\HH^k(X \setminus Y)$. Furthermore, for the same reasons as always, the cup product on the complex $\widetilde{\Omega}_X^\bullet(\log Y)$ is compatible with $F$ and $W$ therefore it induces pairings on the mixed Hodge structure on $\HH^*(X\setminus Y;\mathbb{Q})$.

\begin{defn}
Let $(X,Y)$ be a V-normal crossings pair. We say that an element $\sigma \in \widetilde{\Omega}_X^2(\log Y)$ is vlog symplectic if for each orbifold chart $(Z,D)/G$ of $(X,Y)$, we may find some $\widetilde{\sigma} \in \Gamma(Z,\Omega^2_X(\log Y))^G$ so that $(\rho_*\widetilde{\sigma})^G = \sigma$. If the vlog symplectic form $\sigma$ induces a class in $\HH^2(X \setminus Y;\mathbb{C})$ in $I^{2,0;i}$, we say that $\sigma$ is of pure weight $i$.
\end{defn}
The following result is then analogous to Proposition \ref{prop:mixedis}.
\begin{proposition}
Let $(X,Y)$ be a vlog symplectic pair and $\sigma$ a vlog symplectic form on $(X,Y)$. Then $\HH^*(X\setminus Y;\mathbb{Q})$ is a symplectic Hodge ring. 
\end{proposition}

\begin{example}
Let $(X,Y)$ be a log symplectic pair and let $G$ be a group acting on $X$ which preserves $Y$, and so that all stabilizers of points are small. Assume that there is a log symplectic form $\widetilde{\sigma}$ on which is fixed by $G$. Then $(X,Y)/G$ is a vlog symplectic pair. The most obvious examples of this are symmetric products. Let $(X,Y)$ be a log symplectic pair with log symplectic form $\sigma$. Then $(X,Y)^{\times n}$ with the log symplectic form $\sigma \boxtimes \dots \boxtimes \sigma$ is a log symplectic form as well. The symmetric group $S_n$ acts on $(X,Y)^{\times n}$. The fixed points are the diagonals of $(X,Y)^{\times n}$ and the stabilizers of points are small (since $\dim X \geq 2$). Therefore, the quotient $(X,Y)^{\times n}/S_n$ equipped with the quotient form $\sigma \boxtimes \dots \boxtimes \sigma$ is a vlog symplectic pair.

\end{example}
\end{comment}
